Benchmarking Learnt Radio Localisation under Distribution Shift

Deploying radio frequency (RF) localisation systems invariably entails non-trivial effort, particularly for the latest learning-based breeds. There has been little prior work on characterising and comparing how learnt localiser networks can be deployed in the field under real-world RF distribution shifts. In this paper, we present RadioBench: a suite of 8 learnt localiser nets from the state-of-the-art to study and benchmark their real-world deployability, utilising five novel industry-grade datasets. We train 10k models to analyse the inner workings of these learnt localiser nets and uncover their differing behaviours across three performance axes: (i) learning, (ii) proneness to distribution shift, and (iii) localisation. We use insights gained from this analysis to recommend best practices for the deployability of learning-based RF localisation under practical constraints.

==> tex_content/notations.tex <==
\chapter*{Notations \label{chap:Notations}}

\addcontentsline{toc}{chapter}{Notations}
\markboth{Notations}{Notations}
\setlength\extrarowheight{1em}
\begin{flushleft}
	\begin{longtable}{>{\raggedright}p{0.3\textwidth} >{\raggedright}p{0.69\textwidth}}
	$x$ & scalar variables, especially in time domain: italic lower case letters
	\tabularnewline
	$\mathbf{X}$ & matrix variables: boldface upright upper case letters
	\tabularnewline	
	$x\left(t\right)$ & functions of continuous variables: argument is placed in round parentheses
	\tabularnewline
	$x_{k}$ & scalar elements of a vector or element of a sequence: element index is a subscript
	\tabularnewline
	$X_{ij}$ & scalar elements of a matrix: row and column indices are subscripts
	\tabularnewline
	$\oplus$  & exclusive disjunction (xor)
	\tabularnewline
	$x \ast h $        & convolution of $x$ and $h$
	\tabularnewline
	$P[x<X]$         & probability of $x$ being smaller than $X$
	\tabularnewline
	$\mathbb{E}[X]$         & expected value of $X$
	\tabularnewline
	$\bf{H} \odot \bf{I}$      & Hadamard product of matrix $\bf{H}$ and $\bf{I}$ 
	\tabularnewline
	$j$       & imaginary unit
	\tabularnewline
	$<.>$     & Iverson brackets, turning the statement into Boolean
	\tabularnewline
	$\bf{H}^{\dagger}$ & pseudo inverse of $\bf{H}$
	\end{longtable}
	\par
\end{flushleft}
\setlength\extrarowheight{0em}


==> tex_content/plotcyclelists.tex <==
\pgfplotscreateplotcyclelist{corporate colours markers}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
orange, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
lila, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
hellgrau, mark=text,text mark=p\\%
anthrazit, mark=text,text mark=a\\%
}

\pgfplotscreateplotcyclelist{corporate colours markers double}{%
rot, every mark/.append style={fill=.!80!rot},mark=*\\%
rot, dashed, every mark/.append style={fill=.!80!rot,solid},mark=*\\%
mittelblau, every mark/.append style={fill=.!80!mittelblau},mark=square*\\%
mittelblau, dashed, every mark/.append style={fill=.!80!mittelblau,solid},mark=square*\\%
apfelgruen, every mark/.append style={fill=.!80!apfelgruen},mark=triangle*\\%
apfelgruen, dashed, every mark/.append style={fill=.!80!apfelgruen,solid},mark=triangle*\\%
orange, mark=star\\%
orange, dashed, mark=star\\%
pink, every mark/.append style={fill=.!80!pink},mark=diamond*\\%
pink, dashed, every mark/.append style={fill=.!80!pink,solid},mark=diamond*\\%
violettblau, every mark/.append style={fill=.!80!violettblau},mark=otimes*\\%
violettblau, dashed, every mark/.append style={fill=.!80!violettblau,solid},mark=otimes*\\%
lila, mark=|\\%
lila, dashed, mark=|\\%
gelb, every mark/.append style={fill=.!80!gelb},mark=pentagon*\\%
gelb, dashed, every mark/.append style={fill=.!80!gelb,solid},mark=pentagon*\\%
}
